Astra: Toward General-Purpose Mobile Robots via Hierarchical Multimodal Learning

Modern robot navigation systems encounter difficulties in diverse and complex indoor environments. Traditional approaches rely on multiple modules with small models or rule-based systems and thus lack adaptability to new environments. To address this, we developed Astra, a comprehensive dual-model architecture, Astra-Global and Astra-Local, for mobile robot navigation. Astra-Global, a multimodal LLM, processes vision and language inputs to perform self and goal localization using a hybrid topological-semantic graph as the global map, and outperforms traditional visual place recognition methods. Astra-Local, a multitask network, handles local path planning and odometry estimation. Its 4D spatial-temporal encoder, trained through self-supervised learning, generates robust 4D features for downstream tasks. The planning head utilizes flow matching and a novel masked ESDF loss to minimize collision risks for generating local trajectories, and the odometry head integrates multi-sensor inputs via a transformer encoder to predict the relative pose of the robot. Deployed on real in-house mobile robots, Astra achieves high end-to-end mission success rate across diverse indoor environments.

==> sections/062Experiment_c2.tex <==
% \begin{numberedconclusion}
% \method-Global can adapt to new environment with few to no data.
% \end{numberedconclusion}



% % \begin{table}[h!tbp]
% %     \centering
% %     \footnotesize
% %     %\setlength{\tabcolsep}{10pt} % 增大列间距
% %     \begin{tabular}{lcccc}
% %         \toprule
% %         \multirow{2}{*}{Method}
% %         & \multicolumn{4}{c}{Home} \\
% %         \cmidrule(lr){2-5} % 场景分隔线
% %         & 1m/5°  (\%) & 3°  (\%) & 5° (\%) & 10° (\%) \\
% %         \midrule
% %         MixVPR    & 57.7 & 51.1 & 57.7 & 73.3 \\
% %         Ours (zero-shot)    & 72.7 & 80.0 & 92.7 & 100.0  \\
% %         Ours (few-shot) & 91.1 & 83.4 & 95.3 & 99.4  \\
% %         \bottomrule
% %     \end{tabular}
% %     \caption{Zero-shot/few-shot performance on the home environment}
% %     \label{tab:zero_shot_adaptation}
% % \end{table}

